Hybrid Beamforming for mm-Wave Massive MIMO Systems with Partially Connected RF Architecture

To satisfy the capacity requirements of future mobile systems, under-utilized millimeter wave frequencies can be efficiently exploited by employing massive MIMO technology with highly directive beamforming. Hybrid analog-digital beamforming has been recognised as a promising approach for large-scale MIMO implementations with a reduced number of costly and power-hungry RF chains. In comparison to fully connected architecture, hybrid beamforming (HBF) with partially connected RF architecture is particularly appealing for the practical implementation due to less complex RF power division and combining networks. In this paper, we first formulate single- and multi-user rate maximization problems as weighted minimum mean square error (WMMSE) and derive solutions for hybrid beamformers using alternating optimization. The algorithms are designed for the full-array- and sub-array-based processing strategies of partially connected HBF architecture. In addition to the rate maximizing WMMSE solutions, we propose lower complexity sub-array-based zero-forcing algorithms. The performance of the proposed algorithms is evaluated in two different channel models, i.e., a simple geometric model and a realistic statistical millimeter wave model known as NYUSIM. The performance results of the WMMSE HBF algorithms are meant to reveal the potential of partially connected HBF and serve as upper bounds for lower complexity methods. Numerical results imply that properly designed partially connected HBF has the potential to provide an good compromise between hardware complexity and system performance in comparison to fully digital beamforming.

==> JournalBIB.tex <==
@INPROCEEDINGS{MajidzadehEuCNC, 
	author={M. {Majidzadeh} and A. {Moilanen} and N. {Tervo} and H. {Pennanen} and A. {Tölli} and M. {Latva-aho}}, 
	booktitle={2017 European Conference on Networks and Communications (EuCNC)}, 
	title={Hybrid beamforming for single-user MIMO with partially connected RF architecture}, 
	year={2017}, 
	volume={}, 
	number={}, 
	pages={1-6}, 
	keywords={array signal processing;iterative methods;MIMO communication;singular value decomposition;stochastic processes;wireless channels;hybrid analog-digital beamforming;single-user MIMO system;massive multiple-input multiple-output system;partially connected RF architecture;millimeter-wave technology;partially connected radio frequency architecture;singular value decomposition matching algorithm;SVD algorithm;iterative orthogonalization algorithm;transmit-receive zero forcing algorithm;transmit-receive ZF algorithm;geometry-based stochastic channel model;hybrid precoding;massive MIMO;mm-wave communications;ZF beamforming}, 
	doi={10.1109/EuCNC.2017.7980696}, 
	ISSN={}, 
	month={June},}


@INPROCEEDINGS{MajidzadehPIMRC, 
	author={M. {Majidzadeh} and A. {Moilanen} and N. {Tervo} and H. {Pennanen} and A. {Tolli} and M. {Latva-aho}}, 
	booktitle={2017 IEEE 28th Annual International Symposium on Personal, Indoor, and Mobile Radio Communications (PIMRC)}, 
	title={Partially connected hybrid beamforming for large antenna arrays in multi-user MISO systems}, 
	year={2017}, 
	volume={}, 
	number={}, 
	pages={1-6}, 
	keywords={antenna arrays;array signal processing;diversity reception;MIMO communication;multiuser channels;stochastic processes;multiuser MISO systems;millimeter-wave massive MIMO systems;HBF algorithms;partially connected radio frequency architecture;antenna arrays;maximum ratio transmission beamformer;partially connected hybrid beamforming;digital zero forcing;stochastic channel;subarray-based ZF algorithm;Radio frequency;Antenna arrays;Array signal processing;Optimization;Arrays;MIMO communication;hybrid analog-digital beamforming;massive MIMO;maximum ratio transmission;zero forcing}, 
	doi={10.1109/PIMRC.2017.8292390}, 
	ISSN={2166-9589}, 
	month={Oct},}


@INPROCEEDINGS{MajidzadehSPAWC, 
	author={M. {Majidzadeh} and J. {Kaleva} and N. {Tervo} and H. {Pennanen} and A. {Tölli} and M. {Latva-Aho}}, 
	booktitle={2018 IEEE 19th International Workshop on Signal Processing Advances in Wireless Communications (SPAWC)}, 
	title={Rate Maximization for Partially Connected Hybrid Beamforming in Single-User MIMO Systems}, 
	year={2018}, 
	volume={}, 
	number={}, 
	pages={1-5}, 
	keywords={Radio frequency;Array signal processing;Signal processing algorithms;Optimization;MIMO communication;Antenna arrays;Receiving antennas;hybrid precoding;massive MIMO;mm-wave communications;rate maximization;weighted minimum mean square error}, 
	doi={10.1109/SPAWC.2018.8445883}, 
	ISSN={1948-3252}, 
	month={June},}


@ARTICLE{RXMMMZ, 
	author={T. S. Rappaport and Y. Xing and G. R. MacCartney and A. F. Molisch and E. Mellios and J. Zhang}, 
	journal={IEEE Transactions on Antennas and Propagation}, 
	title={Overview of Millimeter Wave Communications for Fifth-Generation (5G) Wireless Networks -- With a Focus on Propagation Models}, 
	year={2017}, 
	volume={65}, 
	number={12}, 
	pages={6213-6230}, 
	keywords={5G mobile communication;millimetre wave propagation;5G wireless communication systems;fifth generation wireless communication systems;fifth-generation wireless networks;millimeter wave communications;millimeter wave frequency bands;mmWave propagation;propagation models;propagation parameters;unlicensed applications;5G mobile communication;Atmospheric modeling;Computer architecture;Microprocessors;Wireless communication;Wireless fidelity;Cellular network;channel model standards;channel modeling;fifth generation (5G);millimeter wave (mmWave);path loss;propagation}, 
	doi={10.1109/TAP.2017.2734243}, 
	ISSN={0018-926X}, 
	month={Dec},}




@ARTICLE{SR, 
	author={M. K. Samimi and T. S. Rappaport}, 
	journal={IEEE Transactions on Microwave Theory and Techniques}, 
	title={3-D Millimeter-Wave Statistical Channel Model for 5G Wireless System Design}, 
	year={2016}, 
	volume={64}, 
	number={7}, 
	pages={2207-2225}, 
	keywords={5G mobile communication;wireless channels;3D millimeter wave statistical channel model;3D statistical channel impulse response;5G wireless system design;IR model;New York City;angle of arrival power spectra;millimeter wave spectrum;mmWave spectrum;non-LOS channels;ultra-high frequency-microwave;urban line of sight;3GPP;Antenna measurements;Brain modeling;Channel models;Delays;Mathematical model;Mobile communication;28 GHz;3-D ray-tracing;5G;73 GHz;Channel model;impulse response (IR);millimeter-wave (mmWave) propagation;multipath;spatial channel model (SCM);spatial lobe (SL);statistical simulator;time cluster (TC);time cluster spatial lobe (TCSL)}, 
	doi={10.1109/TMTT.2016.2574851}, 
	ISSN={0018-9480}, 
	month={July},}



@ARTICLE{ChenTLHW, 
	author={C. {Chen} and C. {Tsai} and Y. {Liu} and W. {Hung} and A. {Wu}}, 
	journal={IEEE Transactions on Signal Processing}, 
	title={{C}ompressive {S}ensing ({CS}) {A}ssisted {L}ow-{C}omplexity {B}eamspace {H}ybrid {P}recoding for {M}illimeter-{W}ave {MIMO} {S}ystems}, 
	year={2017}, 
	volume={65}, 
	number={6}, 
	pages={1412-1424}, 
	keywords={channel estimation;codecs;compressed sensing;millimetre waves;MIMO communication;precoding;singular value decomposition;compressive sensing assisted low-complexity beamspace hybrid precoding;millimeter-wave MIMO systems;hybrid analog-digital precoding;radio-frequency components;hardware cost reduction;millimeter-wave multiple-input multiple output systems;antenna dimensions;hybrid precoder design;optimal full-digital precoder;hybrid precoder design;beamspace singular value decomposition;reduced-dimension beamspace channel state information;compressive sensing based channel estimators;CS-assisted beamspace hybrid precoding;leverages CS-based CSI;beamspace-SVD reduces complexity;performance loss;optimal full-digital precoder;Radio frequency;Channel estimation;MIMO;Precoding;Matching pursuit algorithms;Complexity theory;Algorithm design and analysis;MIMO;millimeter-wave communication;hybrid precoding;beamforming;low-complexity}, 
	doi={10.1109/TSP.2016.2641379}, 
	ISSN={1053-587X}, 
	month={March},}


@ARTICLE{MirzaANS, 
	author={J. {Mirza} and B. {Ali} and S. {Saud Naqvi} and S. {Saleem}}, 
	journal={IEEE Communications Letters}, 
	title={Hybrid Precoding via Successive Refinement for Millimeter Wave MIMO Communication Systems}, 
	year={2017}, 
	volume={21}, 
	number={5}, 
	pages={991-994}, 
	keywords={Precoding;Radio frequency;Matching pursuit algorithms;Baseband;MIMO;Algorithm design and analysis;Transmitters;MIMO;hybrid beamforming;limited feedback}, 
	doi={10.1109/LCOMM.2017.2655514}, 
	ISSN={1089-7798}, 
	month={May},}


@ARTICLE{ARAPH, 
	author={O. E. Ayach and S. Rajagopal and S. Abu-Surra and Z. Pi and R. W. Heath}, 
	journal={IEEE Transactions on Wireless Communications}, 
	title={{S}patially {S}parse {P}recoding in {M}illimeter {W}ave {MIMO} {S}ystems}, 
	year={2014}, 
	volume={13}, 
	number={3}, 
	pages={1499-1513}, 
	keywords={MIMO communication;array signal processing;millimetre wave antenna arrays;precoding;radio transceivers;RF domain;analog processing;antenna arrays;basis pursuit principle;beamforming gain;cellular systems;hardware limitation;low-cost RF hardware;microwave signals;millimeter wave MIMO systems;millimeter wave signals;mixed-signal devices;mmWave channel spatial structure;mmWave signals;mmWave spectral efficiency;mmWave systems;mmWave transceivers;multiple-data streams;power consumption;precoders;precoding-combining problem;receiver combining;sparse reconstruction problem;spatially sparse precoding;traditional multiantenna systems;transceiver hardware constraint;transmit precoding;unconstrained performance limits;Antenna arrays;Approximation methods;Baseband;Hardware;MIMO;Radio frequency;Vectors;Millimeter wave;antenna arrays;basis pursuit;beamforming;cellular communication;limited feedback;multiple-input multiple-output (MIMO);precoding;sparse reconstruction;sparsity}, 
	doi={10.1109/TWC.2014.011714.130846}, 
	ISSN={1536-1276}, 
	month={March},}



@ARTICLE{ShiRLH, 
	author={Q. Shi and M. Razaviyayn and Z. Q. Luo and C. He}, 
	journal={IEEE Transactions on Signal Processing}, 
	title={{A}n {I}teratively {W}eighted {MMSE} {A}pproach to {D}istributed {S}um-{U}tility {M}aximization for a {MIMO} {I}nterfering {B}roadcast {C}hannel}, 
	year={2011}, 
	volume={59}, 
	number={9}, 
	pages={4331-4340}, 
	keywords={MIMO communication;cellular radio;mean square error methods;optimisation;radio transceivers;MIMO interfering broadcast channel;cellular network;distributed sum-utility maximization;iterative minimization;iteratively weighted MMSE approach;linear beamformers;linear transceiver design algorithm;multiple-input multiple-output interfering broadcast channel;weighted mean-square error;weighted sum-rate maximization problem;Algorithm design and analysis;Covariance matrix;Interference;MIMO;Minimization;Receivers;Transmitters;Linear beamformer;MIMO interfering broadcast channel;sum-utility maximization;weighted MMSE;weighted sum-rate maximization}, 
	doi={10.1109/TSP.2011.2147784}, 
	ISSN={1053-587X}, 
	month={Sept},}


@ARTICLE{ChristensenACC, 
	author={S. S. Christensen and R. Agarwal and E. D. Carvalho and J. M. Cioffi}, 
	journal={IEEE Transactions on Wireless Communications}, 
	title={{W}eighted {S}um-{R}ate {M}aximization {U}sing {W}eighted {MMSE} for {MIMO-BC} {B}eamforming {D}esign}, 
	year={2008}, 
	volume={7}, 
	number={12}, 
	pages={4792-4799}, 
	keywords={MIMO communication;array signal processing;broadcast channels;filtering theory;iterative methods;least mean squares methods;optimisation;MIMO-BC beamforming design;MMSE;iteration method;linear transmit filter design;minimum mean square error method;multiple input multiple output broadcast channel;optimization;weighted sum-rate maximization;Antennas and propagation;Array signal processing;Broadcasting;Downlink;Iterative algorithms;MIMO;Mean square error methods;Meteorological radar;Mutual information;Nonlinear filters;MIMO systems, transceiver design, smart antennas;antennas and propagation.}, 
	doi={10.1109/T-WC.2008.070851}, 
	ISSN={1536-1276}, 
	month={December},}


@ARTICLE{PayamiGD, 
	author={S. {Payami} and M. {Ghoraishi} and M. {Dianati}}, 
	journal={IEEE Transactions on Wireless Communications}, 
	title={Hybrid Beamforming for Large Antenna Arrays With Phase Shifter Selection}, 
	year={2016}, 
	volume={15}, 
	number={11}, 
	pages={7258-7271}, 
	keywords={antenna arrays;array signal processing;phase shifters;Rayleigh channels;hybrid beamforming;antenna arrays;channel matrix;Rayleigh fading;closed-form expression;analog phase shifters;digital phase shifters;power consumption;phase shifter network;wireless channel;spectral efficiency;word length 2 bit;Radio frequency;Phase shifters;Array signal processing;Antenna arrays;Scattering;Receivers;Fading channels;Hybrid beamforming;large MIMO systems;phase shifter selection}, 
	doi={10.1109/TWC.2016.2599526}, 
	ISSN={1536-1276}, 
	month={Nov},}



@ARTICLE{RusuMGH, 
	author={C. {Rusu} and R. {Mèndez-Rial} and N. {González-Prelcic} and R. W. {Heath}}, 
	journal={IEEE Transactions on Wireless Communications}, 
	title={Low Complexity Hybrid Precoding Strategies for Millimeter Wave Communication Systems}, 
	year={2016}, 
	volume={15}, 
	number={12}, 
	pages={8380-8393}, 
	keywords={array signal processing;iterative methods;millimetre wave antenna arrays;MIMO communication;precoding;quantisation (signal);wireless channels;antenna arrays;quantization;optimal digital solution;spectral efficiency;iterative solution;channel state information;analog domain;digital domain;hybrid precoding-combining architecture;digital precoding;beamforming;analog front-end;power consumption;multistream MIMO communication;millimeter wave communication system;low complexity hybrid precoding strategy;Radio frequency;Antenna arrays;MIMO;Precoding;Millimeter wave communication;Algorithm design and analysis;Receiving antennas;Millimeter wave communication;antenna arrays;precoding}, 
	doi={10.1109/TWC.2016.2614495}, 
	ISSN={1536-1276}, 
	month={Dec},}



@ARTICLE{SohrabiYOFDM, 
	author={F. {Sohrabi} and W. {Yu}}, 
	journal={IEEE Journal on Selected Areas in Communications}, 
	title={Hybrid Analog and Digital Beamforming for mmWave OFDM Large-Scale Antenna Arrays}, 
	year={2017}, 
	volume={35}, 
	number={7}, 
	pages={1432-1443}, 
	keywords={array signal processing;broadband networks;millimetre wave antenna arrays;MIMO communication;multi-access systems;OFDM modulation;optimisation;precoding;radio transceivers;wireless channels;hybrid analog and digital beamforming;MM-wave OFDM large-scale antenna arrays;large-scale millimeter wave multiple input multiple output systems;large-scale MM-wave MIMO systems;hardware complexity reduction;frequency-flat channel;broadband MM-wave systems;orthogonal frequency division multiplexing modulation;single-user MIMO system;SU-MIMO system;transmitter;receiver;radio frequency chains;RF chains;transceiver antennas;unified heuristic;spectral efficiency maximization;multiuser multiple input single output case;heuristic hybrid precoding design;weighted sum rate maximisation;Array signal processing;OFDM;Algorithm design and analysis;Antenna arrays;Radio frequency;Precoding;Covariance matrices;Millimeter wave;frequency selective channels;OFDM;large-scale antenna arrays;MIMO;multi-user MISO;massive MIMO;linear beam-forming;precoding;combining}, 
	doi={10.1109/JSAC.2017.2698958}, 
	ISSN={0733-8716}, 
	month={July},}


@ARTICLE{RaghavanSCSKL, 
	author={V. {Raghavan} and S. {Subramanian} and J. {Cezanne} and A. {Sampath} and O. H. {Koymen} and J. {Li}}, 
	journal={IEEE Journal on Selected Areas in Communications}, 
	title={Single-User Versus Multi-User Precoding for Millimeter Wave MIMO Systems}, 
	year={2017}, 
	volume={35}, 
	number={6}, 
	pages={1387-1401}, 
	keywords={channel coding;millimetre waves;MIMO communication;precoding;single-user versus multiuser precoding;millimeter wave MIMO systems;radio frequency chains;multiinput multioutput systems;hybrid precoding;directional precoding structures;robust eigen-mode-based precoding structures;directional structure;single-user precoding schemes;multiuser precoding schemes;multiuser transmissions;RF chain resource;Precoding;MIMO;Radio frequency;Periodic structures;Array signal processing;Antenna arrays;Signal to noise ratio;Millimeter wave;MIMO;beamforming;precoding;single-user MIMO;multi-user MIMO;hybrid precoding;sparse channels}, 
	doi={10.1109/JSAC.2017.2687798}, 
	ISSN={0733-8716}, 
	month={June},}


@ARTICLE{JinZCX, 
	author={J. {Jin} and Y. R. {Zheng} and W. {Chen} and C. {Xiao}}, 
	journal={IEEE Transactions on Wireless Communications}, 
	title={Hybrid Precoding for Millimeter Wave MIMO Systems: A Matrix Factorization Approach}, 
	year={2018}, 
	volume={17}, 
	number={5}, 
	pages={3327-3339}, 
	keywords={matrix decomposition;millimetre wave communication;MIMO communication;optimisation;precoding;millimeter wave MIMO systems;matrix factorization approach;hybrid precoding design;millimeter wave multiple-input multiple-output systems;precoding problem;digital precoders;matrix factorization problem;constant modulus constraints;hybrid precoding schemes;unconstrained optimal precoders;channel matrix;coupled power constraint;hybrid precoding algorithms;Precoding;MIMO communication;Radio frequency;Matching pursuit algorithms;Transmitters;Receiving antennas;Hybrid precoding;finite-alphabet inputs;matrix factorization;nonconvex optimization}, 
	doi={10.1109/TWC.2018.2810072}, 
	ISSN={1536-1276}, 
	month={May},}

@ARTICLE{CaoOS, 
	author={P. L. {Cao} and T. J. {Oechtering} and M. {Skoglund}}, 
	journal={IEEE Communications Letters}, 
	title={Transmit Beamforming for Single-User Large-Scale MISO Systems With Sub-Connected Architecture and Power Constraints}, 
	year={2018}, 
	volume={22}, 
	number={10}, 
	pages={2096-2099}, 
	keywords={antenna arrays;array signal processing;iterative methods;MISO communication;optimisation;precoding;telecommunication power management;optimal phase shift;optimal power allocation;per-antenna power constraints;single-user large-scale MISO systems;subconnected architecture;optimal transmit beamforming;optimal digital precoder;analog precoders;iterative algorithm;maximal power allocation;Radio frequency;Resource management;Transmitting antennas;Array signal processing;Optimization;MISO communication;Large-scale;massive MIMO;sub-connected architecture;hybrid beamforming;per-antenna power constraints}, 
	doi={10.1109/LCOMM.2018.2866265}, 
	ISSN={1089-7798}, 
	month={Oct},}



@INPROCEEDINGS{VlachosKT, 
	author={E. {Vlachos} and A. {Kaushik} and J. {Thompson}}, 
	booktitle={2018 IEEE 87th Vehicular Technology Conference (VTC Spring)}, 
	title={Energy Efficient Transmitter with Low Resolution DACs for Massive MIMO with Partially Connected Hybrid Architecture}, 
	year={2018}, 
	volume={}, 
	number={}, 
	pages={1-5}, 
	keywords={digital-analogue conversion;millimetre wave communication;MIMO communication;optimisation;radio transmitters;telecommunication power management;millimeter wave multiple-input multiple-output systems;future wireless communication standards;mmWave MIMO system components;energy efficient transmitter;mmWave massive MIMO systems;optimization problem;radio-frequency chains;system capacity;energy performance;DAC resolutions;partially connected hybrid architecture;low resolution DAC;beamforming techniques;low resolution digital-to-analog converters;Radio frequency;MIMO communication;Radio transmitters;Energy resolution;Covariance matrices;Power demand}, 
	doi={10.1109/VTCSpring.2018.8417650}, 
	ISSN={2577-2465}, 
	month={June},}


@ARTICLE{LiWLLZ, 
	author={M. {Li} and Z. {Wang} and H. {Li} and Q. {Liu} and L. {Zhou}}, 
	journal={IEEE Wireless Communications}, 
	title={A Hardware-Efficient Hybrid Beamforming Solution for mmWave MIMO Systems}, 
	year={2019}, 
	volume={26}, 
	number={1}, 
	pages={137-143}, 
	keywords={array signal processing;channel estimation;millimetre wave antenna arrays;millimetre wave communication;millimetre wave phase shifters;MIMO communication;precoding;novel hardware-efficient hybrid precoding-combining architecture;spectral efficiency performance;antenna arrays;RF chains;analog precoder-combiner;channel estimation strategy;analog beamformers;high-resolution phase shifters;mmWave communication systems;mmWave MIMO systems;hardware-efficient hybrid beamforming solution;higher energy efficiency;comparable spectral efficiency;hardware-efficient structure;POS-SW-based hybrid beamforming architecture;simple switch network;maximum hardware efficiency;simple phase over-samplers;power consumption;high hardware complexity;Array signal processing;Hardware;Power demand;Radio frequency;Hybrid power systems;MIMO communication;Complexity theory;Millimeter wave communication}, 
	doi={10.1109/MWC.2018.1700391}, 
	ISSN={1536-1284}, 
	month={February},}



@ARTICLE{YuQFJZ, 
	author={H. {Yu} and W. {Qu} and Y. {Fu} and C. {Jiang} and Y. {Zhao}}, 
	journal={IEEE Communications Letters}, 
	title={A Novel Two-Stage Beam Selection Algorithm in mmWave Hybrid Beamforming System}, 
	year={2019}, 
	volume={}, 
	number={}, 
	pages={1-1}, 
	keywords={Measurement;Array signal processing;Radio frequency;Convex functions;Antenna arrays;Precoding;Millimeter wave (mmWave);hybrid beamforming;beam selection;discrete codebook;large-scale antenna array}, 
	doi={10.1109/LCOMM.2019.2913385}, 
	ISSN={1089-7798}, 
	month={},}



@ARTICLE{CastellanosRRKLLP, 
	author={M. R. {Castellanos} and V. {Raghavan} and J. H. {Ryu} and O. H. {Koymen} and J. {Li} and D. J. {Love} and B. {Peleato}}, 
	journal={IEEE Journal of Selected Topics in Signal Processing}, 
	title={Channel-Reconstruction-Based Hybrid Precoding for Millimeter-Wave Multi-User MIMO Systems}, 
	year={2018}, 
	volume={12}, 
	number={2}, 
	pages={383-398}, 
	keywords={array signal processing;feedback;MIMO communication;multiuser channels;precoding;cell-specific codebook;initial beam alignment phase;user-specific codebook;observed signal-to-noise ratio;single-user setting;top-P beam indices;beam weights;multiuser interference;advanced directional precoding structure;receiver beam knowledge;precoder design;hybrid precoding architecture;coarse initial beam alignment codebook;channel-reconstruction;millimeter-wave multiuser MIMO systems;multiuser multiinput multioutput transmissions;multiuser transmissions;base station;beamforming vectors;zero-forcing structure;Structural beams;Radio frequency;Array signal processing;Millimeter wave technology;Antennas;Precoding;Signal to noise ratio;Millimeter wave;multi-input multi-output, multi-user;beamforming;hybrid precoding;phase and amplitude control;zeroforcing;generalized eigenvector;channel estimation}, 
	doi={10.1109/JSTSP.2018.2819135}, 
	ISSN={1932-4553}, 
	month={May},}




@misc{SongKC,
	title={Fully-/Partially-Connected Hybrid Beamforming Architectures for mmWave MU-MIMO},
	author={Xiaoshen Song and Thomas Kühne and Giuseppe Caire},
	year={2019},
	eprint={1904.10276},
	archivePrefix={arXiv},
	primaryClass={cs.IT}
}



@ARTICLE{RatnamMBP, 
	author={V. V. {Ratnam} and A. F. {Molisch} and O. Y. {Bursalioglu} and H. C. {Papadopoulos}}, 
	journal={IEEE Transactions on Signal Processing}, 
	title={Hybrid Beamforming With Selection for Multiuser Massive MIMO Systems}, 
	year={2018}, 
	volume={66}, 
	number={15}, 
	pages={4105-4120}, 
	keywords={antenna arrays;array signal processing;channel estimation;MIMO communication;multi-access systems;radio transceivers;statistical analysis;telecommunication switching;multiuser massive MIMO systems;analog beamforming matrix;L̅ input ports;analog beamformer;average channel statistics;instantaneous channel knowledge;instantaneous channel variations;computational cost;multiuser HBwS system;switch bank architecture;channel estimation overhead;multiuser massive multiple-input-multiple-output systems;hybrid beamforming-with-selection;antenna array;bank-of-switches;up-conversion chains;down-conversion chains;effective analog beams;user separability;beamforming gain;system performance;Array signal processing;Hardware;Channel estimation;MIMO communication;Antenna arrays;Precoding;Beam selection;Antenna selection;mm-wave;Massive MIMO;Beam-space MIMO;Hybrid precoding with selection;Hybrid precoding;Hybrid preprocessing;Grassmannian manifold}, 
	doi={10.1109/TSP.2018.2838557}, 
	ISSN={1053-587X}, 
	month={Aug},}




@ARTICLE{LiHSWM, 
	author={Z. {Li} and S. {Han} and S. {Sangodoyin} and R. {Wang} and A. F. {Molisch}}, 
	journal={IEEE Transactions on Wireless Communications}, 
	title={Joint Optimization of Hybrid Beamforming for Multi-User Massive MIMO Downlink}, 
	year={2018}, 
	volume={17}, 
	number={6}, 
	pages={3600-3614}, 
	keywords={array signal processing;MIMO communication;optimisation;precoding;hybrid beamforming;multiuser massive MIMO downlink;two-stage beamformers;multiuser massive multiple-input multiple-output systems;frequency division duplexing mode;hybrid digital/analog beamforming structures;virtual sectorization;channel-statistics;user grouping;user equipment;intra-group effective channel;channel state information acquisition;Kronecker channel model assumption;optimal analog combiner;intra-group signal;inter-group interference plus noise ratio;digital precoder;geometric-based stochastic models;joint optimization;Radio frequency;Array signal processing;MIMO communication;Training;Interference;Antennas;Downlink;Massive MIMO;FDD;training overhead;hybrid beamforming;virtual sectorization}, 
	doi={10.1109/TWC.2018.2808523}, 
	ISSN={1536-1276}, 
	month={June},}


@ARTICLE{MolischRHLNLH, 
	author={A. F. {Molisch} and V. V. {Ratnam} and S. {Han} and Z. {Li} and S. L. H. {Nguyen} and L. {Li} and K. {Haneda}}, 
	journal={IEEE Communications Magazine}, 
	title={Hybrid Beamforming for Massive MIMO: A Survey}, 
	year={2017}, 
	volume={55}, 
	number={9}, 
	pages={134-141}, 
	keywords={antenna arrays;array signal processing;MIMO communication;transceivers;hybrid beamforming;massive MIMO system;hybrid multiple-antenna transceivers;lower-dimensional digital processing;training overhead;channel state information;signal-to-noise and interference ratio;CSI acquisition;millimeter-wave frequencies;Radio frequency;Array signal processing;MIMO communication;Antennas;NIST;Transceivers;Baseband}, 
	doi={10.1109/MCOM.2017.1600400}, 
	ISSN={0163-6804}, 
	month={Sep.},}



@ARTICLE{RohSPLLKCCA, 
	author={W. Roh and J. Y. Seol and J. Park and B. Lee and J. Lee and Y. Kim and J. Cho and K. Cheun and F. Aryanfar}, 
	journal={IEEE Communications Magazine}, 
	title={Millimeter-Wave Beamforming as an Enabling Technology for {5G} Cellular Communications: Theoretical Feasibility and Prototype Results}, 
	year={2014}, 
	volume={52}, 
	number={2}, 
	pages={106-113}, 
	keywords={anechoic chambers (electromagnetic);array signal processing;cellular radio;millimetre wave propagation;telecommunication traffic;4G cellular networks;5G cellular communications;Korea;United States;anechoic chamber;cellular usage;channel measurement;free space propagation measurements;hybrid beamforming;millimeter-wave beamforming;mobile communications;mobile traffic volume;next generation cellular systems;nonline-of-sight coverage;Antenna arrays;Array signal processing;Millimeter wave communication;Next generation networking;Propagation losses;Prototypes;Radio frequency;Receiving antennas}, 
	doi={10.1109/MCOM.2014.6736750}, 
	ISSN={0163-6804}, 
	month={Feb.},}



@ARTICLE{RappaportSMZAWWSSG, 
	author={T. S. Rappaport and S. Sun and R. Mayzus and H. Zhao and Y. Azar and K. Wang and G. N. Wong and J. K. Schulz and M. Samimi and F. Gutierrez}, 
	journal={IEEE Access}, 
	title={Millimeter Wave Mobile Communications for {5G} Cellular: It Will Work!}, 
	year={2013}, 
	volume={1}, 
	number={3}, 
	pages={335-349}, 
	keywords={broadband networks;cellular radio;directive antennas;millimetre wave propagation;mobile radio;5G cellular;broadband cellular communication network;cellular mm-wave propagation;densely populated indoor environment;densely populated outdoor environment;frequency 28 GHz;frequency 38 GHz;global bandwidth shortage;millimeter wave frequency spectrum;millimeter wave mobile communication;steerable directional antenna;wireless carrier;Base stations;Computer architecture;Directional antennas;MIMO;Microprocessors;Millimeter wave technology;Mobile communication;Wireless communication;28 GHz;38 GHz;5G;MIMO;cellular;channel models;directional antennas;millimeter wave propagation measurements;mobile communications}, 
	doi={10.1109/ACCESS.2013.2260813}, 
	ISSN={2169-3536}, 
	month={May},}


@ARTICLE{LarssonETM, 
	author={E. G. Larsson and O. Edfors and F. Tufvesson and T. L. Marzetta}, 
	journal={IEEE Communications Magazine}, 
	title={Massive {MIMO} for next generation wireless systems}, 
	year={2014}, 
	volume={52}, 
	number={2}, 
	pages={186-195}, 
	keywords={MIMO communication;access protocols;antenna arrays;frequency division multiplexing;ARGOS;MAC layer;frequency-division duplex operation;full-dimension MIMO;hyper MIMO;intentional jamming;large-scale antenna systems;massive MIMO;multiuser MIMO;next generation wireless systems;resource allocation;service antennas;single-antenna terminals;time-division duplex operation;time-frequency bins;very large MIMO;Antenna arrays;Base stations;Downlink;Fading;MIMO;Uplink}, 
	doi={10.1109/MCOM.2014.6736761}, 
	ISSN={0163-6804}, 
	month={Feb.},}


@ARTICLE{RanganRE, 
	author={S. Rangan and T. S. Rappaport and E. Erkip}, 
	journal={Proceedings of the IEEE}, 
	title={Millimeter-Wave Cellular Wireless Networks: Potentials and Challenges}, 
	year={2014}, 
	volume={102}, 
	number={3}, 
	pages={366-385}, 
	keywords={4G mobile communication;antenna arrays;array signal processing;cellular radio;channel capacity;space division multiplexing;4G cellular networks;New York City;adaptive beamforming;adaptive transmissions;carrier aggregation;cellular communication;directional isolation;directional transmissions;frequency 28 GHz;frequency 30 GHz to 300 GHz;heterogeneous network architectures;microcell base station;millimeter-wave cellular wireless networks;multielement antenna arrays;multihop relaying;picocell base station;spatial multiplexing;statistical channel models;Antennas;Atmospheric measurements;Bandwidth;Cellular networks;Millimeter wave communication;Radio spectrum management;Shadow mapping;28 GHz;3GPP LTE;73 GHz;Cellular systems;channel models;millimeter-wave radio;urban deployments;wireless propagation}, 
	doi={10.1109/JPROC.2014.2299397}, 
	ISSN={0018-9219}, 
	month={Mar.},}



@ARTICLE{HanIXRl, 
	author={S. {Han} and C. {I} and Z. {Xu} and C. {Rowell}}, 
	journal={IEEE Communications Magazine}, 
	title={Large-scale antenna systems with hybrid analog and digital beamforming for millimeter wave 5G}, 
	year={2015}, 
	volume={53}, 
	number={1}, 
	pages={186-194}, 
	keywords={array signal processing;cellular radio;channel estimation;energy consumption;millimetre waves;mobile antennas;radio transceivers;large-scale antenna systems;hybrid analog-digital beamforming;millimeter wave 5G;cellular bands;mmWave bands;mobile traffic;energy consumption;digital beamforming structures;analog beamforming structures;transceiver;hybrid beamforming structure;optimal analog beamforming designs;optimal digital beamforming designs;energy efficiency;spectrum efficiency;channel estimation performance;Transceivers;Antennas;Array signal processing;Radio frequency;Downlink;Base stations;5G mobile communication;Millimeter wave communication;Digital communication}, 
	doi={10.1109/MCOM.2015.7010533}, 
	ISSN={0163-6804}, 
	month={January},}



@ARTICLE{ShiH, 
	author={Q. {Shi} and M. {Hong}}, 
	journal={IEEE Journal of Selected Topics in Signal Processing}, 
	title={{S}pectral {E}fficiency {O}ptimization {F}or {M}illimeter {W}ave {M}ultiuser {MIMO} {S}ystems}, 
	year={2018}, 
	volume={12}, 
	number={3}, 
	pages={455-468}, 
	keywords={decomposition;millimetre wave phase shifters;MIMO communication;optimisation;precoding;radio receivers;radio transmitters;spectral efficiency optimization;millimeter wave multiuser MIMO systems;large-scale antenna arrays;power consumption;optimal fully digital precoding;spatial multiplexing gain;optimal hybrid precoding design;nonconvex hybrid precoding problem;mmWave multiuser MIMO systems;penalty dual decomposition method;PDD method;directional beamforming;5G wireless communication;millimeter wave communication;mmWave communication;KKT solution;transmitter;receivers;infinite resolution phase shifter;finite resolution phase shifter;Precoding;Radio frequency;MIMO communication;Optimization;Phase shifters;Array signal processing;Signal processing algorithms;MU-MIMO;mmWave;hybrid precoding;penalty dual decomposition method;BSUM}, 
	doi={10.1109/JSTSP.2018.2824246}, 
	ISSN={1932-4553}, 
	month={June},}




@INPROCEEDINGS{LiN, 
	author={Q. {Li} and H. {Noureddine}}, 
	booktitle={2017 IEEE 28th Annual International Symposium on Personal, Indoor, and Mobile Radio Communications (PIMRC)}, 
	title={Hybrid sum rate maximization beamforming for multi-user massive MIMO millimeter wave system}, 
	year={2017}, 
	volume={}, 
	number={}, 
	pages={1-6}, 
	keywords={millimetre wave communication;MIMO communication;multi-access systems;precoding;multiuser massive MIMO millimeter wave system;two-stage hybrid sum rate maximization precoding algorithm;downlink mmWave multiuser multiple data streams system;radio frequency domain precoder;channel state information;conventional sum rate maximization base band precoding;smaller dimension equivalent user channel;millimeter wave system;two-stage hybrid precoding algorithm;frequency 6.0 GHz;Radio frequency;Array signal processing;Precoding;MIMO communication;Discrete Fourier transforms;Downlink;Optimization}, 
	doi={10.1109/PIMRC.2017.8292253}, 
	ISSN={2166-9589}, 
	month={Oct},}


@ARTICLE{SohrabiY, 
	author={F. {Sohrabi} and W. {Yu}}, 
	journal={IEEE Journal of Selected Topics in Signal Processing}, 
	title={Hybrid Digital and Analog Beamforming Design for Large-Scale Antenna Arrays}, 
	year={2016}, 
	volume={10}, 
	number={3}, 
	pages={501-513}, 
	keywords={array signal processing;cellular radio;millimetre wave antenna arrays;millimetre wave phase shifters;MIMO communication;numerical analysis;power consumption;signal resolution;hybrid digital beamforming design;hybrid analog beamforming design;large-scale antenna array;millimeter wave frequency;mmWave frequency;future wireless cellular communication system;highly directional beamforming;fully digital beamforming method;RF chain component high power consumption;hybrid beamforming architecture;low-dimensional digital beamformer;RF beamformer;analog phase shifter;point-to-point multiple-input multiple-input system;point-to-point MIMO system transmission scenario;downlink multiuser multiple-input single-output system;downlink MU-MISO system transmission scenario;heuristic hybrid beamforming design;finite resolution phase shifter;numerical simulation;Array signal processing;Radio frequency;Antenna arrays;MIMO;Phase shifters;Signal processing algorithms;Millimeter wave;large-scale antenna arrays;multiple-input multiple-output (MIMO);multi-user multipleinput single-output (MU-MISO);massive MIMO;linear beamforming;precoding;combining;finite resolution phase shifters;Combining;finite resolution phase shifters;large-scale antenna arrays;linear beamforming;massive MIMO;millimeter wave;multi-user multiple-input single-output (MU-MISO);multiple-input multiple-output (MIMO);precoding}, 
	doi={10.1109/JSTSP.2016.2520912}, 
	ISSN={1932-4553}, 
	month={April},}



@ARTICLE{UtschickSJL, 
	author={W. {Utschick} and C. {Stöckle} and M. {Joham} and J. {Luo}}, 
	journal={IEEE Transactions on Wireless Communications}, 
	title={Hybrid LISA Precoding for Multiuser Millimeter-Wave Communications}, 
	year={2018}, 
	volume={17}, 
	number={2}, 
	pages={752-765}, 
	keywords={MIMO communication;precoding;signal processing;wireless channels;signal processing;hybrid precoders;linear successive allocation method;low-complexity version;mm-wave channels;hybrid LISA precoding;multiuser millimeter-wave communications;mm-wave frequency bands;antenna elements;base station;power consumption;RF chains;hybrid precoding;Precoding;Antennas;Radio frequency;Equalizers;Algorithm design and analysis;Resource management;Interference;Multiuser communications;mm-wave communications;hybrid precoding;linear successive allocation method;structured mm-wave channels}, 
	doi={10.1109/TWC.2017.2770125}, 
	ISSN={1536-1276}, 
	month={Feb},}



@ARTICLE{WuLY, 
	author={X. {Wu} and D. {Liu} and F. {Yin}}, 
	journal={IEEE Transactions on Communications}, 
	title={Hybrid Beamforming for Multi-User Massive MIMO Systems}, 
	year={2018}, 
	volume={66}, 
	number={9}, 
	pages={3879-3891}, 
	keywords={antenna arrays;array signal processing;channel capacity;MIMO communication;multiple-input multiple-output system;channel state information;HBF systems;base station antenna arrays;channel capacity;communication system;digital precoder/combiner;single cell downlink multiuser massive MIMO system;multiuser massive MIMO systems;hybrid beamforming;Radio frequency;MIMO communication;Baseband;Complexity theory;Antennas;Array signal processing;Channel models;Hybrid beamforming;large scale arrays;MU-MIMO}, 
	doi={10.1109/TCOMM.2018.2829511}, 
	ISSN={0090-6778}, 
	month={Sep.},}



@ARTICLE{ComaUC, 
	author={J. P. {González-Coma} and W. {Utschick} and L. {Castedo}}, 
	journal={IEEE Transactions on Wireless Communications}, 
	title={Hybrid LISA for Wideband Multiuser Millimeter-Wave Communication Systems Under Beam Squint}, 
	year={2019}, 
	volume={18}, 
	number={2}, 
	pages={1277-1288}, 
	keywords={array signal processing;broadband networks;channel coding;computational complexity;millimetre wave communication;OFDM modulation;precoding;radio transmitters;telecommunication scheduling;vectors;wireless channels;uniform linear array steering vectors;hybrid precoders;linear successive allocation;hybrid approach;hybrid LISA;wideband multiuser millimeter-wave communication systems;beam squint;user scheduling;channel frequency selectivity;equivalent narrowband channels;analog preprocessing network;signal bandwidth;hybrid combiners;orthogonal frequency-division multiplexing modulation;precoder-combiner design;OFDM;Wideband;Precoding;Frequency modulation;Interference;Frequency division multiplexing;Millimeter wave;hybrid precoding and combining;wideband;multiuser;MIMO;beam squint;linear successive allocation (LISA)}, 
	doi={10.1109/TWC.2018.2890667}, 
	ISSN={1536-1276}, 
	month={Feb},}



@ARTICLE{KimL, 
	author={M. {Kim} and Y. H. {Lee}}, 
	journal={IEEE Transactions on Vehicular Technology}, 
	title={MSE-Based Hybrid RF/Baseband Processing for Millimeter-Wave Communication Systems in MIMO Interference Channels}, 
	year={2015}, 
	volume={64}, 
	number={6}, 
	pages={2714-2720}, 
	keywords={array signal processing;iterative methods;mean square error methods;MIMO communication;multi-access systems;radiofrequency interference;time-frequency analysis;vectors;RF beamforming vectors;orthogonal-matching-pursuit-based algorithms;minimum-mean-square-error transmit-receive processors;sparse approximation problems;multiuser interference channels;baseband MIMO processor;RF beamformer;radio frequency beamformer;hybrid MIMO processors;hybrid multiple-input multiple-output processor;MIMO interference channels;millimeter-wave communication systems;MSE-based hybrid RF-baseband processing;Radio frequency;MIMO;Vectors;Manganese;Baseband;Interference channels;Approximation methods;Hybrid radio frequency (RF)/baseband processing;mean square error criterion;millimeter-wave (mm-wave) communication;multiple-input multiple-output (MIMO) interference channel;orthogonal matching pursuit (OMP);sparse approximation}, 
	doi={10.1109/TVT.2014.2346400}, 
	ISSN={0018-9545}, 
	month={June},}




@ARTICLE{NguyenLLH, 
	author={D. H. N. {Nguyen} and L. B. {Le} and T. {Le-Ngoc} and R. W. {Heath}}, 
	journal={IEEE Access}, 
	title={Hybrid MMSE Precoding and Combining Designs for mmWave Multiuser Systems}, 
	year={2017}, 
	volume={5}, 
	number={}, 
	pages={19167-19181}, 
	keywords={array signal processing;channel coding;iterative methods;least mean squares methods;MIMO communication;precoding;radio receivers;hybrid MMSE precoding;mmWave multiuser systems;low-complexity alternative;fully digital precoding;millimeter-wave MIMO wireless systems;mixed signal hardware components;hybrid precoding;digital processing;beamforming gains;spatial multiplexing gains;mmWave systems;mean-squared error criteria;analog combiners;hybrid minimum MSE precoder;hybrid precoder;weighted sum-MSE cost function;mmWave channels;design problems;hybrid analog-digital precoding architectures;MMSE precoding-combining;Radio frequency;Precoding;Algorithm design and analysis;Antenna arrays;MIMO;Matching pursuit algorithms;Baseband;Millimeter wave;multiple-input multiple-output (MIMO);antenna arrays;beamforming;precoding;sparse reconstruction;minimum mean squared-error (MMSE)}, 
	doi={10.1109/ACCESS.2017.2754979}, 
	ISSN={2169-3536}, 
	month={},}




@ARTICLE{CongLZ, 
	author={J. {Cong} and T. {Lin} and Y. {Zhu}}, 
	journal={IEEE Communications Letters}, 
	title={Hybrid MMSE Beamforming for Multiuser Millimeter-Wave Communication Systems}, 
	year={2018}, 
	volume={22}, 
	number={11}, 
	pages={2390-2393}, 
	keywords={array signal processing;least mean squares methods;millimetre wave communication;minimisation;multi-access systems;precoding;multiuser millimeter-wave communication systems;minimum mean square error criterion;alternating minimization method;hybrid precoder;base station;BS;hybrid combiners;optimized digital precoder;digital combiners;MMSE HBF scheme;fully digital beamforming;hybrid MMSE beamforming;hybrid analog-and-digital beamforming design;HBF design;closed-form expressions;generalized eigendecomposition;Radio frequency;Array signal processing;MIMO communication;Optimization;Hybrid power systems;Precoding;Multiuser mmWave communication systems;MMSE;HBF;generalized eigen-decomposition}, 
	doi={10.1109/LCOMM.2018.2869329}, 
	ISSN={1089-7798}, 
	month={Nov},}





@ARTICLE{LinCZZB, 
	author={T. {Lin} and J. {Cong} and Y. {Zhu} and J. {Zhang} and K. {Ben Letaief}}, 
	journal={IEEE Transactions on Communications}, 
	title={Hybrid Beamforming for Millimeter Wave Systems Using the MMSE Criterion}, 
	year={2019}, 
	volume={67}, 
	number={5}, 
	pages={3693-3708}, 
	keywords={array signal processing;broadband networks;communication complexity;eigenvalues and eigenfunctions;iterative methods;least mean squares methods;millimetre wave communication;minimisation;telecommunication network reliability;time-frequency analysis;eigenvalue decomposition;hybrid receive beamformers;hybrid transmit beamformers;minimum sum-mean square error criterion;hybrid analog component;hybrid full-digital beamforming;weighted sum-MSE-based design;alternating minimization method;multivariable design problem;broadband mmWave transmissions;HBF design;transmission reliability;power consumption;propagation loss;millimeter-wave communication systems;MMSE criterion;spectral efficiency-based design;alternating minimization algorithms;orthogonal matching pursuit methods;low-complexity general eigenvalue decomposition-based HBF algorithm;computational complexity;constant modulus constraint;manifold optimization-based HBF algorithm;HBF;Array signal processing;Radio frequency;Broadband communication;Matching pursuit algorithms;Optimization;Narrowband;Precoding;Millimeter-wave (mmWave) communications;minimum mean square error (MMSE);hybrid analog and digital beamforming (HBF);alternating optimization;manifold optimization (MO)}, 
	doi={10.1109/TCOMM.2019.2893632}, 
	ISSN={0090-6778}, 
	month={May},}



@ARTICLE{RenWQL, 
	author={Y. {Ren} and Y. {Wang} and C. {Qi} and Y. {Liu}}, 
	journal={IEEE Access}, 
	title={Multiple-Beam Selection With Limited Feedback for Hybrid Beamforming in Massive MIMO Systems}, 
	year={2017}, 
	volume={5}, 
	number={}, 
	pages={13327-13335}, 
	keywords={array signal processing;channel coding;feedback;MIMO communication;optimisation;precoding;Rayleigh channels;statistical analysis;multiple-beam selection method;hybrid analog beamforming;massive digital MIMO system;hybrid multiple-input multiple-output system;5G network;computational complexity;channel state information;zero-forcing precoding;digital beamforming;base station;BS;digital baseband ZF precoding;limited feedback method;Rayleigh fading channel;mmwave channel;Array signal processing;MIMO;Radio frequency;Antennas;Precoding;Interference;Signal to noise ratio;Millimeter wave communication;MIMO;hybrid beamforming;beam selection}, 
	doi={10.1109/ACCESS.2017.2666782}, 
	ISSN={2169-3536}, 
	month={},}




@INPROCEEDINGS{HanifYBSS, 
	author={M. {Hanif} and H. {Yang} and G. {Boudreau} and E. {Sich} and H. {Seyedmehdi}}, 
	booktitle={2016 IEEE Canadian Conference on Electrical and Computer Engineering (CCECE)}, 
	title={Practical hybrid precoding for multi-user massive MIMO systems}, 
	year={2016}, 
	volume={}, 
	number={}, 
	pages={1-4}, 
	keywords={array signal processing;computational complexity;MIMO communication;precoding;hybrid precoding;multiuser massive MIMO systems;sequential-EGT;best-user EGT;equal gain transmission;analog beamforming;analog phased-array;zero-forcing beamforming;interuser interference;Radio frequency;Precoding;Phased arrays;Computer architecture;Array signal processing;Phase shifters;MIMO;Equal-gain transmission;hybrid precoding;spectral efficiency;sub-connected architecture;zero-forcing beamforming}, 
	doi={10.1109/CCECE.2016.7726751}, 
	ISSN={}, 
	month={May},}




@ARTICLE{NohKSL, 
	author={J. {Noh} and T. {Kim} and J. {Seol} and C. {Lee}}, 
	journal={IET Communications}, 
	title={Zero-Forcing Based Hybrid Beamforming for Multi-User Millimeter Wave Systems}, 
	year={2016}, 
	volume={10}, 
	number={18}, 
	pages={2670-2677}, 
	keywords={array signal processing;multi-access systems;multiuser channels;radio transmitters;wireless channels;submission template;zero-forcing-based hybrid beamforming;multiuser millimetre wave system;radiofrequency chain;RF chain;broadband signal power consumption;analogue processing;digital processing;MM-wave beamforming;HBF scheme;multiuser downlink MM-wave system;perfect channel state information at transmitter;CSIT;limited feedback information;multiuser MM-wave channel;sum rate performance enhancement}, 
	doi={10.1049/iet-com.2016.0769}, 
	ISSN={1751-8628}, 
	month={},}




@ARTICLE{HanifYBSSLow, 
	author={M. {Hanif} and H. {Yang} and G. {Boudreau} and E. {Sich} and H. {Seyedmehdi}}, 
	journal={IET Communications}, 
	title={Low-complexity hybrid precoding for multi-user massive MIMO systems: a hybrid EGT/ZF approach}, 
	year={2017}, 
	volume={11}, 
	number={5}, 
	pages={765-771}, 
	keywords={array signal processing;MIMO communication;precoding;radiofrequency interference;singular value decomposition;low complexity hybrid precoding;multiuser massive MIMO systems;hybrid EGT/ZF approach;base station;hybrid precoding design;subconnected analogue;analogue phased arrays;multiuser massive MIMO system;equal gain transmission;EGT;analogue beamforming;analogue phased array;employ zero-forcing;interuser interference;singular value decomposition}, 
	doi={10.1049/iet-com.2016.0983}, 
	ISSN={1751-8628}, 
	month={},}




@INPROCEEDINGS{YuZZ, 
	author={Q. {Yu} and X. {Zhai} and M. {Zhao}}, 
	booktitle={2017 IEEE 86th Vehicular Technology Conference (VTC-Fall)}, 
	title={An Energy-Efficient Hybrid Precoding Algorithm for Multiuser mmWave Massive MIMO Systems}, 
	year={2017}, 
	volume={}, 
	number={}, 
	pages={1-5}, 
	keywords={5G mobile communication;cellular radio;mean square error methods;millimetre wave communication;MIMO communication;multiuser channels;optimisation;precoding;telecommunication power management;transmitting antennas;energy-efficient hybrid precoding algorithm;multiuser mmWave massive MIMO systems;fifth generation cellular networks;radio frequency chains;conventional HP architecture;transmit antennas;energy-efficient weighted minimum mean square error;achievable system sum-rate;RF precoder;RF chain;baseband precoder;WMMSE algorithm;optimal sum-rate performance;digital precoding;analog phase shifters;energy consumption;RF adders;adaptive connection network;partially-connected HP structure;baseband combiner;Radio frequency;Precoding;Algorithm design and analysis;Antennas;MIMO communication;Baseband;Matching pursuit algorithms}, 
	doi={10.1109/VTCFall.2017.8288020}, 
	ISSN={}, 
	month={Sep.},}




@INPROCEEDINGS{LiWHG, 
	author={H. {Li} and T. Q. {Wang} and X. {Huang} and Y. J. {Guo}}, 
	booktitle={2018 IEEE 88th Vehicular Technology Conference (VTC-Fall)}, 
	title={Matrix Normalization Based ZF Hybrid Precoded Multi-User MIMO mmWave Systems with Massive Array}, 
	year={2018}, 
	volume={}, 
	number={}, 
	pages={1-5}, 
	keywords={matrix algebra;millimetre wave antenna arrays;millimetre wave communication;MIMO communication;multi-access systems;precoding;vectors;wireless channels;matrix normalization;ZF hybrid precoded multiuser MIMO;massive array;future wireless communication systems;large-scale antenna arrays;representative hybrid array structures;fully-connected structure;vector normalization;multiuser multiinput-multioutput millimeter wave systems;zero-forcing hybrid precoding;achievable rate upper bound;hybrid array structures;partially-connected structure;Matrix normalization;vector normalization;ZF hybrid precoding;mmWave massive MIMO}, 
	doi={10.1109/VTCFall.2018.8690745}, 
	ISSN={2577-2465}, 
	month={Aug},}




@INPROCEEDINGS{IwanowBU, 
	author={M. {Iwanow} and S. {Bazzi} and W. {Utschick}}, 
	booktitle={WSA 2018; 22nd International ITG Workshop on Smart Antennas}, 
	title={A Greedy Approach for Multiuser mmWave Hybrid Precoding with Subarray Architectures}, 
	year={2018}, 
	volume={}, 
	number={}, 
	pages={1-4}, 
	keywords={}, 
	doi={}, 
	ISSN={}, 
	month={March},}



@ARTICLE{LiWYZY, 
	author={N. {Li} and Z. {Wei} and H. {Yang} and X. {Zhang} and D. {Yang}}, 
	journal={IEEE Access}, 
	title={Hybrid Precoding for mmWave Massive MIMO Systems With Partially Connected Structure}, 
	year={2017}, 
	volume={5}, 
	number={}, 
	pages={15142-15151}, 
	keywords={antenna arrays;MIMO communication;power consumption;precoding;telecommunication power management;water-filling algorithm;optimal digital precoder;single-stream optimal transmitter beamforming problem;signal-to-noise ratio;analog precoder;antenna deployment;optimal hybrid precoder design problem;radio frequency chain;fully connected structure;low power consumption;partially connected structure;millimetre-wave massive MIMO systems;Radio frequency;MIMO;Antenna arrays;Precoding;Optimization;Signal to noise ratio;Massive MIMO;mmWave;hybrid precoder;partially connected structure}, 
	doi={10.1109/ACCESS.2017.2720163}, 
	ISSN={2169-3536}, 
	month={},}



@misc{XingyuLZZ,
	title={{P}artially-{C}onnected {H}ybrid {B}eamforming for {S}pectral {E}fficiency {M}aximization via a {W}eighted {MMSE} {E}quivalence}, 
	author={Xingyu Zhao and Tian Lin and Yu Zhu and Jun Zhang},
	year={2020},
	eprint={2010.04537},
	archivePrefix={arXiv},
	primaryClass={cs.IT}
}



@INPROCEEDINGS{KalevaTJ,
	author={J. {Kaleva} and A. {Tölli} and M. {Juntti}},
	booktitle={2012 IEEE Global Communications Conference (GLOBECOM)}, 
	title={Weighted sum rate maximization for interfering broadcast channel via successive convex approximation}, 
	year={2012},
	volume={},
	number={},
	pages={3838-3843},
	doi={10.1109/GLOCOM.2012.6503715}}

